Elastic Graphs

An elastic graph is a graph with an elasticity associated to each edge. It may be viewed as a network made out of ideal rubber bands. If the rubber bands are stretched on a target space there is an elastic energy. We characterize when a homotopy class of maps from one elastic graph to another is loosening, i.e., decreases this elastic energy for all possible targets. This fits into a more general framework of energies for maps between graphs.

==> Makefile <==
PROJECT= Elastic
SOURCES = $(PROJECT).tex intro.tex basic.tex taut.tex \
	lipschitz.tex harmonic.tex filling.tex energies.tex \
	electrical.tex
BIBSOURCES =  dylan.bib conformal.bib topo.bib graphs.bib
COMMONFILES = defs.tex macros.tex hamsalpha.bst Characterize-v1.aux $(BIBSOURCES)
COMMONDIRS = draws
COMMON = $(COMMONFILES) $(COMMONDIRS)

all: $(PROJECT).pdf

check: check-stamp

check-stamp: figures-stamp $(SOURCES) $(COMMON)
	pdflatex $(PROJECT)
	bibtex $(PROJECT)
	touch check-stamp

$(PROJECT).pdf: $(SOURCES) $(COMMON) figures-stamp
	pdflatex $(PROJECT)
	bibtex $(PROJECT)
	pdflatex $(PROJECT)
	pdflatex $(PROJECT)
	pdflatex $(PROJECT)

$(COMMON): %: ../%
	ln -s ../$@ $@

pack: $(PROJECT).tar.gz

$(PROJECT).tar.gz: $(SOURCES) $(COMMON) $(PROJECT).pdf
	mkdir $(PROJECT) $(PROJECT)/draws
	cp --dereference $(SOURCES) $(COMMONFILES) $(PROJECT).bbl $(PROJECT)/
	cp --dereference $(mpfiles:%=draws/%) $(mpfiles:%.mp=draws/%-*.mps) \
	    draws/macros.mp $(PROJECT)/draws
	cp Makefile $(PROJECT)/
	tar cfvz $(PROJECT).tar.gz $(PROJECT)
	rm -R $(PROJECT)/

# Bits for the drawings
VPATH := ../draws:$VPATH

# MetaPost figures
mpfiles = graphs.mp vertex-tt.mp surface.mp energies.mp weak.mp iter.mp \
	cuts.mp squares.mp reduced.mp
mpsfiles = $(mpfiles:%.mp=%-0.mps)

$(mpsfiles): %-0.mps: %.mp macros.mp
	-find $(<D) -name "$(*F)-[0-9]*.mps" | xargs rm
	-rm $(<D)/"ltx-$(*F).*"
	cd $(<D) && mpost $(<F)
	cd $(<D) && mpost $(<F)

figs = $(mpsfiles)
figures-stamp: $(figs)
	touch figures-stamp

figures: figures-stamp

